FirePower: Towards a Foundation with Generalizable Knowledge for Architecture-Level Power Modeling

Power efficiency is a critical design objective in modern processor design. A high-fidelity architecture-level power modeling method is greatly needed by CPU architects for guiding early optimizations. However, traditional architecture-level power models can not meet the accuracy requirement, largely due to the discrepancy between the power model and actual design implementation. While some machine learning (ML)-based architecture-level power modeling methods have been proposed in recent years, the data-hungry ML model training process requires sufficient similar known designs, which are unrealistic in many development scenarios. This work proposes a new power modeling solution FirePower that targets few-shot learning scenario for new target architectures. FirePower proposes multiple new policies to utilize cross-architecture knowledge. First, it develops power models at component level, and components are defined in a power-friendly manner. Second, it supports different generalization strategies for models of different components. Third, it formulates generalizable and architecture-specific design knowledge into two separate models. FirePower also supports the evaluation of the generalization quality. In our experiments, FirePower can achieve a low error percentage of 5.8% and a high correlation R of 0.98 on average only using two configurations of target architecture. This is 8.8% lower in error percentage and 0.03 higher in R compared with directly training McPAT-Calib baseline on configurations of target architecture.

==> micro_draft_plots/1_OLD_introduction.tex <==


\section{Introduction}
\label{sec:intro}



Stringent energy-efficiency demands drive design decisions across the entire compute-spectrum, ranging from embedded applications, mobile computing to data-centers. As such, accurate power estimation is crucial for making prudent engineering trade-offs not only during CPU microarchitecture design~\cite{haj2016fine,jacobson2011abstraction,zhou2019primal,kim2019simmani} but also for runtime power management such as voltage-noise mitigation and dynamic voltage and frequency scaling (DVFS)~\cite{huang2012accurate,zoni2018powerprobe,reddi2009voltage}. 

{\bf Design-time challenge.}
For design-time power models, a main challenge is how to 
achieve fine-grained resolution with acceptable computation cost. 
CPU design teams typically rely upon industry-standard power analysis tools such as \cite{powerpro} to replay simulation vectors at the RTL or gate-level with back-annotated parasitics. 
Power is computed from the switching statistics of individual signal nets and the capacitive load that they drive. 
This approach is very accurate and serves as the signoff standard, but it comes with a very high computational cost. For instance, generating a power trace of 20 cycles for a power-virus benchmark on the Arm{\textsuperscript{\textregistered}} Neoverse{\texttrademark} N1 microprocessor~\cite{arm-neoverse-n1, christy20208} requires approximately an hour of execution time on a modern high-performance computing (HPC) cluster machine. Clearly, such an approach does not scale for analyses that require long-running workloads and/or simultaneous execution of multiple CPU cores. 

An alternative approach relies upon FPGA-based netlist emulation~\cite{emulation-platform} to address the speed impact of power estimation. In this approach, a simulation trace is generated from FPGA and the extracted switching statistics are then processed using power analysis EDA software~\cite{powerpro} to obtain power traces. 
However, per-cycle power tracing is still onerous using this approach due to the significant storage constraints on modern computer servers. 
Our own benchmarking studies demonstrate storage requirements in excess of 200GB for a 17-million cycle simulation, leading to infeasible execution time using power analysis tools. Thus, this approach is typically restricted to coarse-grained temporal resolution where power tracing is averaged over millions of CPU cycles.


\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{_fig/introductory.pdf}
\vspace{-.1in}
\caption{APOLLO provides a design-time power simulator and a runtime on-chip power meter (OPM) based on a consistent model, as an example, for Neoverse{\texttrademark} N1.}
\vspace{-.2in}
\label{introduct}
\end{figure}  



\begin{table*}[th!]
  \centering
        \vspace{-.1in} \hspace{-.15in}
  \resizebox{1.02\linewidth}{!}{ \renewcommand{\arraystretch}{1.2} 
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{\multirow{2}{*}{Methods (Hardware Overhead in Area \%)}}  &  \textbf{Demonstrated}  & \textbf{Model}   & \textbf{Temporal} & \textbf{\multirow{2}{*}{PC / Proxy Selection}}  & \textbf{Cost or}  \\
     &    \textbf{Application}   &  \textbf{Type}            &  \textbf{Resolution}  &    & \textbf{Overhead} \\
    \hline
    \hline
    CA News00\cite{brooks2000wattch}, HPCA11\cite{jacobson2011abstraction}, OSR06\cite{lee2006accurate}, MICRO09\cite{li2009mcpat},  RAPIDO14\cite{rethinagiri2014system}  \ 
                & \multirow{3}{*}{Design-time}   & \multirow{1}{*}{Analytical}   & \multirow{1}{*}{>1K cycles} &  \multirow{1}{*}{N/A}   &   \multirow{1}{*}{Low}  \\
    %MICRO09\cite{li2009mcpat},  RAPIDO14\cite{rethinagiri2014system}  &  &  &   &   &\\
    \cline{1-1} \cline{3-6} 
    DAC20\cite{zhang2020grannite}  \
                &     & \multirow{4}{*}{Proxies}       & \multirow{2}{*}{>1K cycles}   &  \multirow{4}{*}{Automatic}  &  High \\
    \cline{1-1}  \cline{6-6}
    TODAES00\cite{bogliolo2000regression}, ISCA14\cite{shao2014aladdin}    \ 
                &  software model    &    &   &   & Medium \\
    \cline{1-1} \cline{4-4} \cline{6-6} 
    DAC19\cite{zhou2019primal}  \
                &        &        & \multirow{2}{*}{Per-cycle}   &   &   High \\
    \cline{1-1} \cline{6-6}
    IBM J03\cite{brooks2003new}, DATE15\cite{lee2015dynamic}, MLCAD19\cite{kumar2019learning}, DAC00\cite{ye2000design}, VLSI98\cite{wu1998cycle}  \
                &     &        &         &        &   Medium \\
    \hline
    \hline
    DAC05\cite{coburn2005power} \ \ \textbf{(300\%)}  &  \multirow{3}{*}{Design-time}  &  \multirow{4}{*}{Proxies}  &  \multirow{2}{*}{Per-cycle} &   \multirow{3}{*}{Automatic} &  High  \\
     \cline{1-1} \cline{6-6}
     
   ASPDAC15\cite{yang2015early} \ \ \textbf{(16\%)} \  %ghodrat2007accelerating, coburn2005power
                &    \multirow{3}{*}{FPGA emulation}   &        &      &    &  \multirow{3}{*}{Medium}  \\

    \cline{1-1} \cline{4-4}
    MICRO19\cite{kim2019simmani}     &        &       & $\sim$100s cycles  &    &  \\
    \cline{1-1} \cline{4-5}
    FPL10\cite{sunwoo2010presto}   &     &        &  Per-cycle  &  Hybrid manual/auto   &   \\
    \hline
    \hline
    EW00\cite{bellosa2000benefits}, ICS10\cite{bertran2010decomposable}, ISPASS07\cite{bircher2007complete}, ISLPED05\cite{gilberto2005power}, IGCC10\cite{goel2010portable}, \           &  \multirow{6}{*}{Runtime monitor}   & \multirow{4}{*}{PC}     & \multirow{3}{*}{>1K cycles}   &   \multirow{4}{*}{Manual}  &   \multirow{4}{*}{Low}  \\
     MICRO12\cite{huang2012accurate}, MICRO03\cite{isci2003runtime}, ISLPED01\cite{JosephISLPED01}, DATE15\cite{oboril2015high}, CASES13\cite{pricopi2013power}, &   &   &   &  &  \\
     TCAS-II13\cite{rodrigues2013study}, TCAD20\cite{sagi2020lightweight}, CA News09\cite{singh2009real}, TCAD16\cite{walker2016accurate} &   &   &   &  & \\
    \cline{1-1} \cline{4-4} 
    ISQED17\cite{kalyanam2017power} \ 
                &      &       & $\sim$100s cycles    &         &     \\
    \cline{1-1} \cline{3-5} \cline{6-6}
    TCAD17\cite{najem2016design} \textbf{(1.5-4\%)}, DATE18\cite{pagliari2018all} \textbf{(7\%)}, SUSCOM20\cite{cremona2020automatic} \textbf{(2-20\%)} \
                &      & \multirow{2}{*}{Proxies}      & >1K cycles   & \multirow{2}{*}{Automatic}  &   \multirow{2}{*}{Medium}  \\
    \cline{1-1} \cline{4-4} 
         MIC'PRO18\cite{zoni2018powertap} \textbf{(4-10\%)}, DATE18\cite{zoni2018powerprobe} \textbf{(7\%)}   \
                &     &       & $\sim$100s cycles  &    &   \\
    \hline
    \hline
    \multirow{2}{*}{APOLLO \ \ \  \textbf{(0.2\% overhead)} }   \
                & Design-time model     & \multirow{2}{*}{Proxies}      & \multirow{2}{*}{Per-cycle}  &  \multirow{2}{*}{Automatic}  & \multirow{2}{*}{Low}\\
                & Runtime monitor    &         &           &        &  \\
    \hline
  \end{tabular}
  } 
  \vspace{-.1in}
  \caption{Comparison among various power modeling approaches. The percentage numbers are area overheads.}
      \label{prev_works}
      \vspace{-.15in}
\end{table*}







{\bf Runtime challenge.}
%The requirements on power estimation differ according to the targeted design problem. 
A chief challenge for runtime power model/monitoring is how
to obtain fine-grained resolution with negligible hardware overhead. At runtime, DVFS is orchestrated by the system firmware and/or the operating system (OS), and hence only require coarse-grained power tracing extending over epochs that are milliseconds in duration. In contrast, assessing the throughput impact of CPU pipeline features such as adaptive-clocking~\cite{mair2017adaptiveclocking,bowmanJSSCAdaptiveClocking} and instruction-issue throttling requires power traces at per-cycle granularity. Such pipeline features are typically deployed to address voltage droops due to $Ldi/dt$ transients~\cite{webel2020proactive}, which develop in $<10$ cycles in modern CPU designs. Hence, assessing the performance impact of these micro-architectural features requires fine-grained power tracing capabilities.
% \footnote{Adaptive-clocking~\cite{mair2017adaptiveclocking,bowmanJSSCAdaptiveClocking} and issue throttling are typically deployed to address timing emergencies due to $L\frac{di}{dt}$ transients~\cite{webel2020proactive}. Voltage-droop due to these transients develop in $<10$ cycles in modern CPU designs. Hence, assessing the performance impact of these micro-architectural features requires fine-grained power tracing capabilities.}


In the prior art, several works have demonstrated runtime regression models using hardware performance counters (PCs) to guide OS-orchestrated DVFS~\cite{JosephISLPED01, bircher2007complete, walker2016accurate}. These models average counter-values that accumulate PC events, such as L2 cache misses and the number of retired instructions, across thousands (or millions) of CPU cycles. However, averaging over long periods renders these approaches inaccurate when fine-grained power tracing is required. 
In addition, PC-based models are typically developed based on knowledge of a specific well-studied microprocessor and thus cannot be automatically applied to novel CPU designs, which leads to extra engineering cost and longer design time. 
%Thus, existing approaches for power estimation lead to undesirable trade-offs between accuracy and speed that render them unsuitable for fine-grained  power estimation.  

Recently, RTL-based runtime power monitoring with on-chip power meter (OPM) 
\cite{najem2016design,cremona2020automatic,pagliari2018all,
zoni2018powerprobe, zoni2018powertap} have been proposed to improve temporal resolution at the cost of dedicated hardware circuit. However, existing techniques struggle to simultaneously achieve high resolution and low hardware area overhead. For example, 
the work of \cite{najem2016design} restricts area overhead
to 1.5-4\%, but its highest temporal resolution is 2500 clock cycles, which is still quite coarse-grained. A recent work~\cite{zoni2018powertap} improves resolution to 100 cycles, but its area overhead increases to 4-10\%, which is significant enough for raising concerns regarding practicality. 

%bridge the gap between the conflicting demands of temporal resolution and computational speed. Most of these approaches use non-linear mathematical models for improved accuracy, which are further prototyped using FPGAs for runtime monitoring. However, their hardware implementation cost is not explicitly optimized towards a practical on-chip model on ASIC. For this reason, developing fine-grained practical OPMs for arbitrary CPU cores is desired for architects. For example, the work of \cite{najem2016design} (\cite{zoni2018powertap}) achieves $1.5-4\%$ ($4-10$\%) area overhead, but its temporal resolution is around $2500$ (100) clock cycles.
%However, their hardware implementation cost is not explicitly optimized towards a practical on-chip model on ASIC and they are not demonstrated on industry-standard CPU cores. 



%Thus, an automated fine-grained power framework for both design trade-off and runtime throughput controlling is desired for future architecture research. 



We propose APOLLO, a unified RTL power modeling framework addressing both the design-time and runtime challenges with a consistent model structure. Its overview is provided in Figure~\ref{introduct}. The centerpiece of APOLLO is a new power proxy selection technique based on minimax concave penalty (MCP) regression. 
%for both design-time microarchitecture optimization and runtime power monitoring on ASIC as shown 
%After power proxy selection, the accuracy of APOLLO model is further improved by retraining with a ridge regression method.
%We demonstrate the compatibility of APOLLO with emulator-assisted power analysis flow enabling per-cycle power tracing for benchmarks running over millions of CPU cycles. 
%At microarchitecture design time, 
%It achieves high accuracy with temporal resolution of single clock cycles. For design-time power modeling, 
%The light-weighted APOLLO model can be integrated with emulator-assisted power analysis, 
It enables per-cycle power tracing for benchmarks running over millions of CPU cycles.
For runtime monitoring, it provides cycle-accuracy with $<0.2\%$ area overhead. To the best of our knowledge, APOLLO is the first power monitoring technique with cycle-accuracy and sub-$1\%$ area overhead. Moreover, the proxy selection process in APOLLO is fully automated and thereby can be easily applied to any new architectures.
Compared to PRIMAL~\cite{zhou2019primal}, a recent machine learning approach, APOLLO reaches similar accuracy but is orders of magnitude faster. APOLLO also significantly outperforms Simmani~\cite{kim2019simmani}, another state-of-the-art work, on both accuracy and computation speed. Moreover, APOLLO achieves both finer-granularity and lower hardware overhead than \cite{pagliari2018all}, a recent OPM technique.
%Furthermore, the APOLLO power model is efficiently synthesized into an OPM with negligible area and power overheads. 

%We summarize our main contributions of this work as follows:
Our main contributions in APOLLO are as follows:
\begin{itemize}
    \item \textbf{Fine-Granularity Low-Overhead OPM:} APOLLO provides the first runtime OPM that simultaneously achieve per-cycle temporal resolution and $<1\%$ area overhead without compromising accuracy. %which guides CPU pipeline features for voltage droop mitigation. 
    %It is also generalized for any size of power measurement windows to support various design trade-offs or runtime power managements.
    %\item \textbf{Low-Overhead Runtime OPM:} A low-overhead OPM is optimized towards a practical implementation on the Neoverse N1 microprocessor. With $<0.1\%$ accuracy loss from weight quantization, the OPM is prototyped under the state-of-the-art 7nm technology with only $<0.2\%$ of the total area of the core. 
    \item \textbf{Automation:} The overall framework automatically generates training data, develops the model, and constructs the OPM for an arbitrary novel CPU core with minimum designer interference. This reduces the engineering cost and design time on power estimation. 
    %\item \textbf{Light-Weighted Model at Design-Time:} By selecting a very small number of proxies with MCP, the APOLLO model is light-weighted. Integrated with \seqsplit{emulator-assisted} power analysis, it generates per-cycle power traces spanning 17 million cycles in minutes. 
    \item \textbf{Validation on Representative Designs:} APOLLO is verified on industry-standard CPU cores with millions of gates, namely, Arm{\textsuperscript{\textregistered}} Neoverse{\texttrademark} N1~\cite{arm-neoverse-n1} microprocessor and Cortex{\textsuperscript{\textregistered}}-A77 \cite{arm-cortex-a77-trm} microprocessor. Neoverse N1 builds cloud-to-edge infrastructure at world-class performance, and Cortex-A77 targets mobile and laptop devices with high energy efficiency. APOLLO achieves an \(R^2 > 0.95\) by monitoring \(< 0.1 \%\) of the RTL signals on both microprocessors. 
    \item \textbf{Light-Weighted Model at Design-Time:} The light-weighted APOLLO model finishes per-cycle power estimation on millions-of-cycles benchmarks in minutes when integrated in \seqsplit{emulator-assisted} power analysis. It allows architects  examine the whole real-world workloads with extremely low cost.
    % on every design specification. 
    %\item \textbf{Unified Framework:} APOLLO is a unified power modeling framework that performs both design-time power simulation and runtime on-chip power monitoring with a consistent model structure. 
    %\item We present APOLLO, the first unified per-cycle power modeling method that performs both design-time power simulation and runtime on-chip power monitoring with a consistent model structure. It is further generalized for the power of any size of power measurement window.
    %Central to APOLLO is the Minimax Concave Penalty (MCP) algorithm that performs power proxy selection.
    %\item We present a highly automated flow to develop the APOLLO model and runtime OPM on ASIC for an arbitrary novel CPU core with minimum designer interference. This flow includes the auto-generation of diverse micro-benchmarks on the given design as the training data.   
    %\item We demonstrate APOLLO on industry-standard CPU cores, namely, Arm{\textsuperscript{\textregistered}} Neoverse{\texttrademark} N1~\cite{arm-neoverse-n1} and Cortex{\textsuperscript{\textregistered}}-A77 \cite{arm-cortex-a77-trm} microprocessors, achieving an \(R^2 > 0.95\) by monitoring the toggling activities of \(< 0.1 \%\) of the RTL signals. 
    %\item We integrate APOLLO into the emulator-assisted power analysis flow for large-scale benchmarks, generating per-cycle power traces spanning 17 million cycles within minutes.
    %\item We demonstrate a low-overhead APOLLO-based on-chip power meter (OPM) for runtime power monitoring. It is optimized towards a practical implementation on the Neoverse N1 microprocessor. With $<0.1\%$ accuracy loss from weight quantization, the OPM is prototyped under the state-of-the-art 7nm technology with $<0.2\%$ of the total area of the core. 
    %With $<0.1\%$ accuracy loss from weight quantization, the OPM is prototyped under the state-of-the-art 7nm technology with $<0.2\%$ of the total area of the Neoverse N1 microprocessor.
\end{itemize}




\section{Related Work}


%Power modeling is an extensively studied topic. 
We summarize representative power estimation approaches in Table \ref{prev_works}. In general, they can be categorized into: 1) design-time power models; 2) runtime on-chip power monitors. 


\subsection{Design-time Power Models}

%Power modeling approaches are employed at design-time to estimate power dissipation during design-space exploration. 
At design-time, chip power dissipation is estimated at architecture or RTL levels for design space exploration. Many approaches~\cite{brooks2000wattch,li2009mcpat,lee2006accurate,jacobson2011abstraction, rethinagiri2014system} construct analytical models for micro-architectural power estimation by collecting statistics from performance simulators~\cite{binkert2011gem5, binkert2006m5}. 
Wattch~\cite{brooks2000wattch} is an architectural dynamic power simulation tool using a linear model, and McPAT~\cite{li2009mcpat} further integrates power, area, and timing in its modeling framework. However, these models typically only estimate an average power over thousands or millions of clock cycles. 
In addition, significant inaccuracies have been observed~\cite{xi2015quantifying, lee2015powertrain, rethinagiri2014system} for McPAT, a well-known model, on new processor designs. To reduce such errors, significant engineering effort~\cite{xi2015quantifying,lee2015powertrain} is required from experienced designers. 
%To alleviate the error, designers are suggested to carefully tune  parameters, perform low-level power validation~\cite{xi2015quantifying}, or even train a calibration model with measurements from real hardware~\cite{lee2015powertrain}. 


Another type of design-time power models are built upon RTL proxies, which are a limited number of selected RTL signals. 
Such models are employed to perform software simulations on cluster machines to estimate power according to signal transitions of the proxies. 
Some early works~\cite{bogliolo2000regression, wu1998cycle, ye2000design} construct macro-models to abstract power estimate for small circuit modules with thousands of gates annotated with parasitics. 
In recent years, machine learning (ML) techniques are exploited to accelerate power estimate computing. Lee, et al.~\cite{lee2015dynamic} adopt non-linear gradient boosting and Kumar, et al.~\cite{kumar2019learning} apply an individual decision tree model to every component of a simple microprocessor design. PRIMAL~\cite{zhou2019primal} predicts per-cycle power by processing transitions of all registers with convolutional neural network (CNN). GRANNITE~\cite{zhang2020grannite} makes use of graph convolutional network~\cite{kipf2017semi} to estimate the average power of each workload. Although these ML techniques achieve significant speedup compared with accurate commercial tools~\cite{powerpro}, it still takes a prohibitively long inference time to perform per-cycle simulation for large-scale benchmarks on industry-standard CPU designs. Evidently, these techniques are too costly for on-chip monitoring.
%In comparison, APOLLO identifies a small number of most relevant proxies and builds a highly light-weighted model. This whole process, including training benchmarks generation, is fully automatic for any novel hardware designs without designer expertise.  


FPGA emulation~\cite{coburn2005power, kim2019simmani, yang2015early, sunwoo2010presto} is a popular approach to accelerating power simulations for large designs. Please note that the term ``emulation'' here is in a broad sense to cover any use of FPGA at design-time. In reality, there are various ways to do so, which may be named differently in other literature. Perhaps the first power emulation work is \cite{coburn2005power}, which has 300\% hardware overhead. Another work~\cite{yang2015early} employs singular value decomposition (SVD), which is computationally expensive. 
Both \cite{coburn2005power} and \cite{yang2015early} are demonstrated only at block-level designs. A microprocessor level application of FPGA emulation is Simmani~\cite{kim2019simmani}, whose temporal resolution is 128 clock cycles. PrEsto~\cite{sunwoo2010presto} achieves cycle-accuracy, but its hardware cost is quite significant, e.g., it consumes more than 50\% of LUTs on Xilinx Virtex-5 LX330 to simulate ARM Cortex-A8 processor design. 
Moreover, its proxy selection process is not completely automated.

%The hardware overhead of the model can be excessive, reaching 300\%~\cite{coburn2005power}. The work in~\cite{yang2015early} performs singular value decomposition (SVD) on all register signals, and Simmani~\cite{kim2019simmani} adopts polynomial combinations of all selected RTL proxies in the model on FPGA. These operations are costly without careful optimization although their overheads are not disclosed. It shall be noted that these emulation approaches are different from the emulator-assisted power estimation proposed in Section~\ref{sec:intro}, which only extracts switching statistics from netlist emulation, then feeds them into power analysis software~\cite{powerpro} or power models to generate power traces.





\subsection{Runtime On-Chip Power Meters (OPMs)}
% not-manual \cite{walker2016accurate, gilberto2005power}
% manual     \cite{, }


%Runtime power modeling is the other key application of power estimation. The runtime power can be directly measured with analog sensors~\cite{bhagavatula2012low, bhagavatula2013power}. A common sensor measures the voltage drop due to a current load and provide the proportional measurement on current consumption. It typically requires an extra analog-to-digital converter (ADC) to map the measurement to a digital output, which brings significant hardware overhead. Thus there is a growing interest in indirect measurement through power models. 

Analog power sensors~\cite{bhagavatula2012low, bhagavatula2013power} can provide accurate
power estimate at runtime. However, they entail ADCs, which imply large area overhead.
A popular runtime approach is to
estimate power dissipation according to 
performance counters (PCs)~\cite{bellosa2000benefits, bircher2007complete,bertran2010decomposable, goel2010portable, huang2012accurate, isci2003runtime, JosephISLPED01, pricopi2013power, rodrigues2013study, singh2009real, sagi2020lightweight, walker2016accurate, gilberto2005power}. Since PCs already exist in most microprocessor designs, they can be treated as free and the associated area overhead is the minimum.    %have been proposed to monitor runtime power. By accumulating selected hardware events, these models are implemented on chip with low hardware cost. 
However, PC-based methods typically rely on architects' knowledge of a specific design to define representative hardware events. 
%This limits transferring existing methods from already well-studied microprocessors to novel designs. 
This limits existing methods to well-studied microprocessors and hinders automatic migration to new designs.
For example, \cite{isci2003runtime, bellosa2000benefits, bircher2007complete} target only Intel Pentium{\textsuperscript{\textregistered}} processors, \cite{kalyanam2017power} is only for the Qualcomm Hexagon 680 DSP, and both works of \cite{pricopi2013power} and \cite{walker2016accurate} are geared toward ARM Cortex-A7 and Cortex-A15 processors. 
Moreover, PC-based power monitors are usually restricted to coarse-grained temporal resolutions, e.g., hundreds or thousands of clock cycles.

%\cite{huang2012accurate} is only for IBM Power7
%In addition, limited by the temporal granularity of PMC events, these models only provide coarse-grained runtime estimations for OS-level power or thermal management. Exceptions include the work of~\cite{kalyanam2017power}, which enables window sizes in hundreds of cycles for power management~\cite{kalyanam202135} and voltage droop mitigation~\cite{kalyanam2020proactive} on Qualcomm Hexagon 680 DSP.  


%Some works~\cite{sunwoo2010presto} still require manual selection. Compared with ASIC, FPGA allows a much higher hardware implementation overhead, and most proxies-based models are prototyped on it. The work in~\cite{yang2015early} performs singular value decomposition (SVD) on all register signals on FPGA. Simmani~\cite{kim2019simmani} adopts polynomial combinations of all selected RTL proxies in their runtime model, which is validated on FPGA. These operations may be too costly and require extra engineering effort in hardware optimization if implemented on ASIC. 


Compared to PC-based techniques, proxy-based power monitors are much more friendly to automatic 
development~\cite{najem2016design,cremona2020automatic,pagliari2018all,zoni2018powerprobe, zoni2018powertap}. 
However, they need more dedicated circuits and
therefore cause more significant area overhead.
Existing proxy-based techniques mostly struggle between low overhead and fine temporal resolution. Some of them \cite{najem2016design, cremona2020automatic, pagliari2018all} are coarse-grained with temporal resolution of thousands of cycles. Their area overhead ranges
from 1.5\% to 20\%. A key reason for the limited resolution is that the proxy selection in many previous methods still has significant room for improvement. For example, the proxy selection in \cite{pagliari2018all} is based on Lasso and our results indicate that APOLLO provides much higher accuracy than Lasso-based technique.
%However, many works~\cite{najem2016design, cremona2020automatic, pagliari2018all} require a higher hardware overhead than PMC-based methods without providing a better temporal resolution. The work of~\cite{najem2016design} adopts several traditional ML techniques, work of~\cite{cremona2020automatic} groups signals with similar activities, and work of~\cite{pagliari2018all} selects proxies with Lasso regression. They update power estimation every thousands of cycles, with area overheads ranging from $1.5\%$ to $20\%$. 
Recent methods~\cite{zoni2018powerprobe, zoni2018powertap} improve  temporal resolution to 100 cycles. To limit extra overhead from improved resolution, they restrict all proxies to primary I/O signals of design modules, which significantly reduce the freedom of proxy selection as well as the underlying model for power monitors. Even with this restriction, their area overhead is still $>4\%$~\cite{zoni2018powerprobe, zoni2018powertap}. In \cite{kalyanam2020proactive}, a digital power meter technique is introduced for handling voltage droop in DSP processors. 
This technique takes advantage of predictable dataflow patterns, which rarely exist in general purpose microprocessors.
In \cite{webel2020proactive}, power proxies are assisted by critical path monitors to obtain fine-grained power monitoring. The area cost of critical path monitors is usually quite significant. 
%Efficient runtime models targeting ASIC strictly require low hardware implementation overhead. To reduce the overhead, models in~\cite{pagliari2018all} produce a new power estimation every few thousand cycles. It selects proxies with Lasso regression~\cite{tibshirani1996regression}, which proves inefficient in our experiment. 


%In comparison, APOLLO provides the first per-cycle power tracing OPM with an extremely low overhead $<0.2\%$, which is $>20\times$ lower than previous OPMs with fine resolution. %For an arbitrary novel design, the OPM is developed by simply configuring generic high-level synthesis (HLS) templates, requiring minimum designer effort. %We also generalize the APOLLO to any size of a power measurement window with high accuracy. 


%In summary, APOLLO is a unified per-cycle power modeling framework for both design-time power simulation and runtime power monitoring. It is not straightforward to handle both tasks efficiently with a consistent model. Most design-time models, designed for high accuracy when executed on HPC clusters, will cause extraordinarily high overhead if implemented on hardware. For runtime models, their efficiency-accuracy trade-off is neither optimized for nor verified on design-time applications. For example, the runtime model performing SVD~\cite{yang2015early} may be optimized to achieve acceptable efficiency on FPGA, but it is too slow for per-cycle simulation on large-scale benchmarks, while being outperformed in accuracy by CNN-based design-time models~\cite{zhou2019primal}. Detailed comparisons are shown in Section~\ref{sec:results}.

\subsection{Position of APOLLO}

%Although proxy-based techniques have been intensively studied, APOLLO distinguishes itself from previous methods by its high effective proxy selection technique. APOLLO provides the first proxy-based OPM approach with area overhead $<1\%$. APOLLO is the first OPM technique that can simultaneously achieves cycle-accuracy and $<1\%$ area overhead without compromising accuracy. APOLLO is also a unified framework that can be applied for both FPGA-based power emulation and OPM. For design-time applications, APOLLO enables cycle-accurate power estimation for millions of clock cycles of traces within several minutes. This is not obviously achievable by any published previous work.   

Although proxy-based techniques have been intensively studied, APOLLO distinguishes itself from previous methods by its highly effective proxy selection technique.
APOLLO is the first fully-automated framework that simultaneously achieves accurate power-estimation with per-cycle temporal granularity and generates low-cost silicon implementation with $<1\%$ of area overhead. 
For design-time applications, APOLLO enables cycle-accurate power estimation for millions of clock cycles of traces within several minutes. This is not obviously achievable by any published previous work. Furthermore, APOLLO is proven on commercial million-gate microprocessor designs (Arm Neoverse N1 and A77 CPU cores) shipping in high-volume, thus indicating scalability to real-world applications in power-management. 
By contrast, many recent works are validated only on small designs, e.g., 80K-gate RISC-V core~\cite{zhou2019primal,zhang2020grannite} and block level designs~\cite{pagliari2018all,yang2015early,zoni2018powertap,zoni2018powerprobe}.



%It is not a simple task to directly apply design-time models during runtime, and vice versa.  
%In addition, we provide an accurate extension of APOLLO for any size of a timing measurement window. 


%Many proxies-based models are implemented on FPGA, which has generally lower requirement on hardware cost than ASIC. 

%Depending on the implementation cost


%Based on design and technology parameters,~\cite{brooks2000wattch,li2009mcpat,lee2006accurate} generate power models to provide unit-level power breakdown for system-level design space exploration.
%The works of~\cite{bellosa2000benefits,bircher2007complete,bertran2010decomposable,walker2016accurate} use performance counters to estimate runtime power for driving OS-level power and thermal management.
%For RTL and netlist-level power analysis, emulation platforms have been adopted in~\cite{ghodrat2007accelerating,coburn2005power,sunwoo2010presto} for large-scale benchmarks to generate power estimations using the calibrated power models prototyped on the same emulator infrastructure.
%It shall be noted that these approaches are different from the emulator-assisted power estimation in Section~\ref{sec:intro}, which extracts switching statistics from netlist emulation and feeds them into power analysis software~\cite{powerpro} to generate power traces.
%Recently, machine learning (ML) models are proposed to perform both fast design-time power simulation and runtime power monitoring at the RTL level. 
%PRIMAL~\cite{zhou2019primal} is a design-time solution, which adopts various deep learning techniques for improved power prediction accuracy. 
%GRANNITE~\cite{zhang2020grannite} proposes a graph-based learning technique to estimate the averaged power.
%The work of \cite{yang2015early} applies singular value decomposition to reduce the model complexity. 
%Power proxy selection approaches have been employed in the past~\cite{huang2012accurate,yang2015early,zhou2019primal,kim2019simmani,kumar2019learning}. 
%Some of them are based on manual selection~\cite{huang2012accurate,kumar2019learning}, while others simply take flip-flop signals as power proxies~\cite{yang2015early,zhou2019primal}. 
%However, the number of flip-flops is not small enough to generate a low-cost OPM for large-scale designs. 
%Compared to the clustering-based method for power proxy selection in~\cite{kim2019simmani}, APOLLO not only improves accuracy but also reduces model complexity from quadratic to linear. 



